The centralizers of root subgroups in Kac-Moody Steinberg groups

For the affine and hyperbolic root system the symmetric part of the centralizers of root subgroups in the corresponding Steinberg groups are calculated. In the affine case the corresponding root subsystems can be computed in term of the centralizers in the spherical root systems, while in the hyperbolic case there emerges a "zoo" of examples, many of them non-hyperbolic. This also delivers many examples of naturally occuring root subsystems of infinite rank.

==> tikzlibrarymultiplebond.code.tex <==
\tikzset{
    triple/.style={
        preaction={preaction={draw,double distance=7},draw}
    }
}

\tikzset{
    quadruple/.style={
        preaction={preaction={draw,double distance=10}},draw,double distance=3
    }
}   
